Open Multiparty Sessions

Multiparty sessions are systems of concurrent processes, which allow several participants to communicate by sending and receiving messages. Their overall behaviour can be described by means of global types. Typable multiparty session enjoy lock-freedom. We look at multiparty sessions as open systems by a suitable definition of connection transforming compatible processes into gateways (forwarders). A relation resembling the standard subtyping relation for session types is used to formalise compatibility. We show that the session obtained by connection can be typed by manipulating the global types of the starting sessions. This allows us to prove that lock-freedom is preserved by connection.

==> eptcsdata.tex <==
\providecommand{\firstpage}{77}
\providecommand{\publicationstatus}{M. Bartoletti, L. Henrio, A. Mavridou, A. Scalas (Eds.):\\
12th Interaction and Concurrency Experience (ICE 2019).\\
EPTCS 304, 2019, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.304.6}{10.4204/EPTCS.304.6}}

